Solving Forward and Inverse Problems of Contact Mechanics using Physics-Informed Neural Networks

This paper explores the ability of physics-informed neural networks (PINNs) to solve forward and inverse problems of contact mechanics for small deformation elasticity. We deploy PINNs in a mixed-variable formulation enhanced by output transformation to enforce Dirichlet and Neumann boundary conditions as hard constraints. Inequality constraints of contact problems, namely Karush-Kuhn-Tucker (KKT) type conditions, are enforced as soft constraints by incorporating them into the loss function during network training. To formulate the loss function contribution of KKT constraints, existing approaches applied to elastoplasticity problems are investigated and we explore a nonlinear complementarity problem (NCP) function, namely Fischer-Burmeister, which possesses advantageous characteristics in terms of optimization. Based on the Hertzian contact problem, we show that PINNs can serve as pure partial differential equation (PDE) solver, as data-enhanced forward model, as inverse solver for parameter identification, and as fast-to-evaluate surrogate model. Furthermore, we demonstrate the importance of choosing proper hyperparameters, e.g. loss weights, and a combination of Adam and L-BFGS-B optimizers aiming for better results in terms of accuracy and training time.

==> sections/introduction/intro_1_motivation.tex <==
\subsection{Motivation}\label{sec1_1}
\ifhidden
{}
\else
\mytodo{
\begin{itemize}
    \item you have already an intro, use some parts to start
    \item What drives us in terms of PINNs? 
    \begin{itemize}
        \item Fast-to-evaluate model
        \item Mesh-free
        \item Easy integration of data
        \item Inverse problem
    \end{itemize}
    \item What drives us in terms of PINNs for contact mechanics? 
\end{itemize}
}
\fi

==> sections/introduction/intro_2_litera.tex <==
\subsection{Literature Review}\label{sec1_2}
\ifhidden
{}
\else
\mytodo{
Literature review of PINNs, particularly on
\begin{itemize}
    \item PINNs on Solid mechanics 
    \item PINNs on elastoplasticity --> KKT
\end{itemize}
}
\fi

==> sections/introduction/intro_3_novelty.tex <==
\subsection{Scientific Novelty and Limitations}\label{sec1_3}

\ifhidden
{}
\else
\mytodo{
\begin{itemize}
    \item Emphasize
    \begin{itemize}
        \item First in contact mechanics
        \item Complementarity functions instead of sign and sigmoid
    \end{itemize}
    \item Limitations
    \begin{itemize}
        \item General limitations of PINNs:
        \begin{itemize}
            \item convergence, 
            \item initial guess for network parameters,
            \item complexity of the model,
            \item choosing the correct hyperparameters.
        \end{itemize}
        \item Finding contact pairs in contact between elastic-elastic domains
        \item Limited to small deformation and 2D
    \end{itemize}
\end{itemize}
}
\fi

==> sections/introduction/intro_4_organizations.tex <==
\subsection{Paper Organization}\label{sec1_4}
\ifhidden
{}
\else
\mytodo{
\begin{itemize}
    \item Tell what will happen in each section
\end{itemize}
}
\fi

==> sections/problem_formulation/contact_m.tex <==
\subsection{Contact mechanics}\label{sec2_2}

Under the assumption of linear elasticity, the governing equations of contact mechanics problems 
involve the classical set of \textit{Karush-Kuhn-Tucker} (KKT) constraints, commonly also referred to 
as \textit{Hertz-Signorini-Moreau} (HSM) conditions and the frictionless sliding condition expressed as
\begin{align}
    \label{eq:gn}
    g_n & \geqslant 0, \\
    \label{eq:pn}
    p_n & \leqslant 0, \\
    \label{eq:gn_pn}
    p_n g_n & =0, \\
    \label{eq:tn}
    t_{\tau} & =0.
\end{align}

\afterequation
Here, $g_n$ is the gap between two bodies in the normal direction and Eq. \ref{eq:gn} pertains to 
the kinematic aspects of non-penetration as shown in Fig. \ref{fig:contact_illus}. 
If two bodies are in contact, the gap vanishes i.e. $g_n=0$. The term $p_n$ denotes 
the normal component of contact traction, namely contact pressure. Correspondingly, 
Eq. \ref{eq:pn} means that no adhesive stresses are allowed in the contact zone which ensures that 
two bodies remain in contact. Furthermore, the complementarity requirement in Eq. \ref{eq:gn_pn} necessitates that the gap should be zero 
when there is a non-zero contact pressure (active set of points),  
and the contact pressure should be zero if there is a positive gap (inactive set of points). 
The complementarity requirement distinguishes an active and inactive set of points. 
It should be noted that the tangential component of the traction vector vanishes for frictionless contact, resulting in Eq. \ref{eq:tn}. 
For additional information regarding contact constitutive laws, 
refer to \cite{popp2012mortar, laursen2003computational, wriggers2006computational, kikuchi1988contact}. 

\begin{figure}[thbp]
    \centering
    \def\dist{\hspace*{5.25cm}}
    \stackinset{c}{-0.2in}{b}{-0.25in}{(a) \dist (b) \dist (c)}{
    \includegraphics[scale=0.625]{contact_configuration_2-eps-converted-to.pdf} 
    } 
    \caption{Demonstration for the two-body finite deformation contact problem. 
    (a) Reference configuration, (b) current configuration, 
    (c) accompanying boundary conditions, illustration of the gap, tangential traction and contact pressure.}
    \label{fig:contact_illus}
\end{figure}

The gap function $g_n$ is defined as a distance measure between the contact boundaries of two bodies
in the current configuration as 
\begin{equation}
    g_n = -\boldsymbol{n}\cdot[\boldsymbol{x^{(1)}}-\boldsymbol{\hat x^{(2)}}]
\end{equation}

\afterequation
with
\begin{equation}
    \label{eq:displacementvector}
    \boldsymbol{u^{(i)}} = \boldsymbol{x^{(i)}} - \boldsymbol{X^{(i)}}
\end{equation}

\afterequation
Here, $\boldsymbol{X}$ represents the reference configuration while $\boldsymbol{x}$ is the current configuration 
(see Fig. \ref{fig:contact_illus}a).
The $\boldsymbol{\hat x^{(2)}}$ term denotes the projection of $\boldsymbol{x^{(1)}}$ onto the surface of $\Omega^{(2)}$ 
(see , Fig. \ref{fig:contact_illus}b).
Furthermore, the $p_n$ and $t_{\tau}$ terms can be obtained by decomposing contact traction as

\begin{equation}
    \label{eq:contact_traction1}
    \boldsymbol{\hat t}_c=p_n \boldsymbol{n}+t_{\tau} \boldsymbol{\tau}, \quad p_n=\mathbf{\hat t}_c \cdot \boldsymbol{n}, \quad t_{\boldsymbol{\tau}}=\boldsymbol{\hat t}_c \cdot \boldsymbol{\tau},
\end{equation}

\afterequation
where 
\begin{equation}
    \label{eq:contact_traction2}
    \boldsymbol{\hat t}_c=\boldsymbol{\sigma}_c\cdot \boldsymbol{n} \quad\quad \text{on }  \partial \Omega_C.
\end{equation}

\afterequation
The term $\boldsymbol{n}$ denotes the outward unit normal and $\boldsymbol{\tau}$ is the unit tangential 
on the slave contact boundary $\partial \Omega_C$ in the reference configuration. Similar to the Neumann boundary condition,
Cauchy's law states that contact stress tensor $\boldsymbol{\sigma_c}$ maps the normal vector 
to the contact boundary $\partial \Omega_C$ to the traction vector $\boldsymbol{\hat t}_c$.
Note that boundary normal vector $\boldsymbol{n}$ can be computed on the reference configuration assuming 
small strain theory (linear elasticity).

==> sections/problem_formulation/lin_elas.tex <==
\subsection{Solid mechanics: Linear elasticity}\label{sec2_1}
Let us consider the equations of boundary value problem (BVP) in linear elasticity

\begin{align}
    \label{eq:lin_equi}
    \boldsymbol{\nabla \cdot \sigma} + \boldsymbol{b} & = \boldsymbol{0} \quad\quad \text{in }  \Omega, \\ %, \quad\quad \text{in }  \Omega
    \boldsymbol{u} &=\boldsymbol{\hat u} \quad\quad \text{on } \partial \Omega_D, \nonumber \\ %\quad\quad \text{on }  , \partial \Omega_D
    \boldsymbol{\sigma} \cdot \mathbf{n} &=\boldsymbol{\hat t} \quad\quad \text{on }  \partial \Omega_N \nonumber, %\quad\quad \text{on },  \partial \Omega_N
\end{align}

\afterequation
where $\boldsymbol{\sigma}$ denotes the Chauchy stress tensor, $\boldsymbol{b}$
presents the body force and $\boldsymbol{u}$ is the displacement vector
which is the primal variable and $\boldsymbol{n}$ is the unit outward 
normal. Prescribed displacements are presented by 
$\boldsymbol{\hat u}$ on the Dirichlet boundary $\partial \Omega_D$  and $\boldsymbol{\hat t}$ denotes
prescribed tractions on the Neumann boundary $\partial \Omega_N$. 

Equations expressing the kinematic relation
and constitutive model or Hooke's law for linear elasticity are, respectively,

\begin{align}
    \label{eq:compatibility}
    \bm{\varepsilon} &= \frac{1}{2}(\boldsymbol{\nabla}\boldsymbol{u}+\boldsymbol{\nabla}\boldsymbol{u}^T), \\
    \label{eq:hooke}
    \boldsymbol{\sigma} &= \mathbb{C} : \bm{\varepsilon}.
\end{align}

\afterequation
Here, $\bm{\varepsilon}$ is the infinitesimal strain tensor and $\mathbb{C}$ is the elasticity tensor.
In the specific case of linear isotropic elasticity, Hooke's law can be expressed as

\begin{equation}
    \boldsymbol{\sigma} = \lambda tr(\bm{\varepsilon})\mathbf{I}+2\mu\bm{\varepsilon},
\end{equation}

\afterequation
where $\lambda$ and $\mu$ are the Lam\'e parameters, $tr(\cdot)$ is the \textit{trace} operator to sum strain 
components on the main diagonal and $\mathbf{I}$ is the identity matrix. 



